Lithium and Beryllium in NGC 752 -- An Open Cluster Twice the Age of the Hyades

The surface abundances of the light elements lithium (Li) and beryllium (Be) reveal information about the physical processes taking place in stellar interiors. The investigation of the amount of these two elements in stars in open clusters shows the effect of age on those mechanisms. We have obtained spectra of both Li and Be in main-sequence stars in NGC 752 at high spectral resolution and high signal-to-noise ratios with HIRES on the Keck I telescope. In order to make meaningful comparisons with other clusters, we have determined the stellar parameters on a common scale. We have found abundances of Li and Be by spectral synthesis techniques. NGC 752 is twice the age of the well-studied Hyades cluster. We find that 1) The Li dip centered near 6500 K is wider in NGC 752, having expanded toward cooler temperatures; 2) The Be dip is deeper in the older NGC 752; 3) The Li "peak" near 6200 K is lower by about 0.3 dex; 4) Although there is little Be depletion in the cooler stars, it is possible that Be may be lower in NGC 752 than in the Hyades; 5) The Li content in both clusters declines with decreasing temperature, but there is less Li in NGC 752 at a given temperature by $\sim$0.4 dex. These differences are consistent with the transport of the light-element nuclei below the surface convection zone as predicted by theory. That connection to rotational spin-down is indicated by the pattern of rotation with temperature in the two clusters.

==> authors.tex <==
\author[0000-0002-8468-9532]{Ann Merchant Boesgaard}
\affiliation{Institute for Astronomy, University of Hawai`i, 2680 Woodlawn Drive, Honolulu, HI 96822, USA}

\author[0000-0001-7205-1593]{Michael G. Lum}
\affiliation{Institute for Astronomy, University of Hawai`i, 2680 Woodlawn Drive, Honolulu, HI 96822, USA}

\author[0000-0003-1125-2564]{Ashley Chontos}
\altaffiliation{NSF Graduate Research Fellow}
\affiliation{Institute for Astronomy, University of Hawai`i, 2680 Woodlawn Drive, Honolulu, HI 96822, USA}

\author[0000-0002-3854-050X]{Constantine P. Deliyannis}
\affiliation{Department of Astronomy, Indiana University, 727 East 3rd Street, Bloomington, IN 47405-7105, USA}
